YASO: A Targeted Sentiment Analysis Evaluation Dataset for Open-Domain Reviews

Current TSA evaluation in a cross-domain setup is restricted to the small set of review domains available in existing datasets. Such an evaluation is limited, and may not reflect true performance on sites like Amazon or Yelp that host diverse reviews from many domains. To address this gap, we present YASO - a new TSA evaluation dataset of open-domain user reviews. YASO contains 2,215 English sentences from dozens of review domains, annotated with target terms and their sentiment. Our analysis verifies the reliability of these annotations, and explores the characteristics of the collected data. Benchmark results using five contemporary TSA systems show there is ample room for improvement on this challenging new dataset. YASO is available at https://github.com/IBM/yaso-tsa.

==> old/3_comprehensive_labeling_analysis_table.tex <==
\newcommand{\targetsPercentageColumnTitle}[0]{\columnTitle{TC}}
\newcommand{\validTargetsPercentageColumnTitle}[0]{\columnTitle{C}}
\newcommand{\numAnnotatorsColumnTitle}[0]{\columnTitle{A}}

\begin{table*}[t]
\tabcolsep=0.1cm
\begin{center}
\begin{tabular}{lcccccccccccc}
\toprule
& 
\multicolumn{2}{c}{\bf \textit{Amazon}} & \multicolumn{2}{c}{\bf \textit{Opinosis}} & \multicolumn{2}{c}{\bf \textit{SST}} & \multicolumn{2}{c}{\bf \textit{Yelp}} & \multicolumn{2}{c}{\bf \textit{SE14-L}} & \multicolumn{2}{c}{\bf \textit{SE14-R}}
\\
\cmidrule(rl){2-3}
\cmidrule(rl){4-5}
\cmidrule(rl){6-7}
\cmidrule(rl){8-9}
\cmidrule(rl){10-11}
\cmidrule(rl){12-13}
\bf \numAnnotatorsColumnTitle & 
\targetsPercentageColumnTitle & \validTargetsPercentageColumnTitle & 
\targetsPercentageColumnTitle & \validTargetsPercentageColumnTitle & 
\targetsPercentageColumnTitle & \validTargetsPercentageColumnTitle & 
\targetsPercentageColumnTitle & \validTargetsPercentageColumnTitle & 
\targetsPercentageColumnTitle & \validTargetsPercentageColumnTitle & 
\targetsPercentageColumnTitle & \validTargetsPercentageColumnTitle 
\\
\midrule
%% start of automatic table
\textbf{1} & \percentage{58.3} & \percentage{43.8} & \percentage{57.5} & \percentage{60.6} & \percentage{62.7} & \percentage{43.7} & \percentage{60.4} & \percentage{46.2} & \percentage{53.8} & \percentage{65.9} & \percentage{53.6} & \percentage{71.6}
\\
\textbf{2} & \percentage{23.4} & \percentage{86} & \percentage{21.6} & \percentage{91.8} & \percentage{19.3} & \percentage{90.2} & \percentage{22.1} & \percentage{94.2} & \percentage{13.9} & \percentage{77.3} & \percentage{10} & \percentage{72}
\\
\textbf{3} & \percentage{11.4} & \percentage{96.3} & \percentage{12.9} & \percentage{98.2} & \percentage{11.8} & \percentage{96.2} & \percentage{10.2} & \percentage{98.7} & \percentage{10.8} & \percentage{100} & \percentage{12.8} & \percentage{100}
\\
\textbf{4} & \percentage{4.8} & \percentage{100} & \percentage{5.2} & \percentage{100} & \percentage{5.1} & \percentage{98.5} & \percentage{5} & \percentage{98.6} & \percentage{13.9} & \percentage{100} & \percentage{18.4} & \percentage{100}
\\
\textbf{5} & \percentage{2.1} & \percentage{100} & \percentage{2.5} & \percentage{100} & \percentage{1.1} & \percentage{100} & \percentage{2.4} & \percentage{100} & \percentage{7.6} & \percentage{100} & \percentage{5.2} & \percentage{100}
%%% end of automatic table
\\
\bottomrule
\end{tabular}
\end{center}
\caption{An analysis of the sentiment label selected in the first and second annotation phases.
For each \emph{\textbf{dataset}} the table shows (i) the percentage of target candidates (\targetsPercentageColumnTitle) identified by multiple annotators (\numAnnotatorsColumnTitle) in the first annotation phase; the percentage of the \targetsPercentageColumnTitle candidates that their first phase sentiment was verified as correct in the second phase (\validTargetsPercentageColumnTitle). See \sectionRef{section:annotation_analysis}.}
\label{tab:comprehensive_labeling_analysis} 
\end{table*}

==> old/6_baselines.tex <==
\section{Baseline Systems}

To establish benchmark results on the new data, the following five \TSAtaskName systems were reproduced using their available codebases.
\\
\listItem{\href{https://github.com/IMPLabUniPr/BERT-for-ABSA}{\baselineNameBAT}} \cite{karimi2020adversarial}:
A pipelined system with domain-specific language models \citep{xu-etal-2019-bert} augmented with  adversarial data.
\\
\listItem{\href{https://github.com/yangheng95/LCF-ATEPC}{\baselineNameLCF}} \cite{yang2020multitask}:  
A joint model based on BERT-SPC, a BERT sentence pair classification model adapted to \ABSAtaskName in \citet{DBLP:journals/corr/SongAEN19}, with domain adaptation and a local context focus mechanism.
\\
\listItem{\href{https://github.com/NLPWM-WHU/RACL}{\baselineNameRACL}} \cite{chen-qian-2020-relation}:
An end-to-end multi-task learning and relation propagation system. We used the RACL-GloVe variant, based on pre-trained word embeddings. 
\\
\listItem{\href{https://github.com/lixin4ever/BERT-E2E-ABSA}{\baselineNameBERTEE}} \cite{li-etal-2019-exploiting}: 
A BERT-based end-to-end system of sequence labeling with a unified tagging scheme. We used the simplest architecture of a linear classification layer for the downstream model.
\\
\listItem{\baselineNameHASTASC}
A pipeline of two systems: (i) \href{https://github.com/lixin4ever/HAST}{HAST} -- Truncated History-Attention (THA) and Selective Transformation Network (STN), for capturing aspect detection history and opinion summary \citep{li-etal-2018-aspect}
(ii) \href{https://github.com/xuuuluuu/Aspect-Sentiment-Classification}{MCRF-SA} -- multiple CRF-based structured attention model for extracting aspect-specific opinion spans and then sentiment classification \citep{xu-etal-2020-aspect}.

\input{tables/6_baseline_results}

==> old/datasets_usage_table.tex <==
\newcommand{\used}[0]{+}
\newcommand{\notUsed}[0]{-}

\newcommand{\recentWork}[8]{
%\multirow{#1}{*}{\parbox{2.3cm}{#2}} &
\multirow{#1}{*}{#3} &
\multirow{#1}{*}{#4} &
\multirow{#1}{*}{#5} &
\multirow{#1}{*}{#6} &
\multirow{#1}{*}{#7} &
\multirow{#1}{*}{\parbox{6cm}{#8}} 
\\}
\newcommand{\emptyLine}[0]{& & & & & \\}

\begin{table*}%[t]
\tabcolsep=0.10cm
%\small
\begin{center}
%\renewcommand*{\arraystretch}{0.93}
\begin{tabular}{lccccl}
\toprule
%\bf Venue &
\bf Work &
\bf \SeLapName &
\bf \SeResName &
\bf \semEvalOneFiveName & 
\bf \semEvalOneSixName &
\bf Additional datasets
\\
\midrule

%%%% 2020 %%%%

% BAT
\recentWork{1}{Arxiv}{\citet{karimi2020adversarial}}{\used}{\used}{\notUsed}{\used}{---}
%Lap: ATE and ASC. 
%\\ Res: \SeLapName for AE,\semEvalOneSixName for ASC.}
%\emptyLine
% LCF
\recentWork{1}{Arxiv}{\citet{yang2020multitask}}{\used}{\used}{\notUsed}{\notUsed}{Chinese reviews data\citep{yang2020multitask}.}
% MCRF
\recentWork{1}{EMNLP 2020}{\citet{xu-etal-2020-aspect}}{\used}{\used}{\used}{\used}{---}
%
\recentWork{3}{EMNLP 2020}{\citet{gong-etal-2020-unified}}{\used}{\used}{\used}{\used}{Device reviews
 \citep{toprak-etal-2010-sentence}, and web service reviews \citep{hu2004mining}.}
\emptyLine
\emptyLine
%
\recentWork{1}{EMNLP 2020}{\citet{xu-etal-2020-aspect}}{\used}{\used}{\used}{\used}{---}
%
\recentWork{1}{LREC 2020}{\citet{rietzler-etal-2020-adapt}}{\used}{\used}{\notUsed}{\notUsed}{---}
%RACL
\recentWork{2}{ACL 2020}
{\citet{chen-qian-2020-relation}}
{\used}{\used}{\used}{\notUsed}
{Opinion term labels \cite{wang2016recursive,wang2017coupled}}
\emptyLine
% SKEP
\recentWork{1}{ACL 2020}{\citet{tian-etal-2020-skep}}{\used}{\used}{\notUsed}{\notUsed}{---}
%sun-etal-2019-utilizing, DBLP:journals/corr/SongAEN19, zeng-LCF-2019, phan-ogunbona-2020-modelling
% BERT-E2E

%%%% 2019 %%%%

\recentWork{1}{W-NUT @EMNLP 2019}
{\citet{li-etal-2019-exploiting}}
{\used}{\used}{\used}{\used}
{}%Data follows \citet{li2019unified}.}
%\emptyLine
%
\recentWork{1}{ACL 2019}
{\citet{ma-etal-2019-exploring}}
{\used}{\notUsed}{\notUsed}{\used}
{---}
%
\recentWork{1}{AAAI 2019}
{\citet{li2019unified}}
{\used}{\used}{\used}{\used}
{%Res: Unified all SE datasets. Also 
Tweets \citep{mitchell-etal-2013-open}.}
%\emptyLine
% BERT-PT
\recentWork{1}{NACCL 2019}{\citet{xu-etal-2019-bert}}{\used}{\used}{\notUsed}{\used}{---}
% \cite{li-lu-2019-learning}
% HAST
\recentWork{1}{IJCAI 2018}
{\citet{li-etal-2018-aspect}}
{\used}{\used}{\used}{\used}
{---}
%tang-etal-2016-effective, tang-etal-2016-aspect, ruder-etal-2016-hierarchical, Ma2018TargetedAS,  DBLP:conf/sbp-brims/HuangOC18, He2018EffectiveAM
\bottomrule
\end{tabular}
\end{center}
\caption{A survey of the evaluation datasets used (marked as \textbf{\used}) within a sample of recent works.}
\label{tab:datasets_usage} 
\end{table*}

